A limit theorem for generalized tempered stable processes and their quadratic variations with stable index tending to 2 and its application to finance

We investigate the joint limiting behavior of a multidimensional Generalized Tempered Stable (GTS) process and its quadratic covariation as the stable index tends to two. Under appropriate scaling, the GTS process converges to a Brownian motion, while its renormalized covariation process converges to an independent stable process with stable index one. As an application, we construct a pure-jump perturbation model around the Black-Scholes model and derive an asymptotic expansion of the at-the-money implied volatility skew.

==> settings/layout_en.tex <==
% Visual layout only. No mathematical notation is defined here.

\geometry{
    top=20mm,
    bottom=25mm,
    left=20mm,
    right=20mm
}

\titleformat*{\section}{\LARGE\bfseries}
\titleformat*{\subsection}{\Large\bfseries}
\titleformat*{\subsubsection}{\large\bfseries}

% Title position and font; keep the main file's \title{...} content-only.
\RequirePackage{etoolbox}
\newlength{\TitleVerticalOffset}
\setlength{\TitleVerticalOffset}{-10mm}
\newcommand{\TitleFont}{\bfseries}
\makeatletter
\patchcmd{\@maketitle}{\@title}
    {\vspace{\TitleVerticalOffset}{\TitleFont\@title}}
    {}{\PackageError{layout_en}{Could not apply title layout}{Check the document class definition of \string\@maketitle.}}
\makeatother

% Match the compact list indentation in layout_jp (one em per nested level).
\setlist[itemize]{leftmargin=1em,labelsep=4.5pt}
\setlist[itemize,1]{leftmargin=2em,label=$\bullet$}
\setlist[itemize,2]{label=$\circ$}
\setlist[itemize,3]{label=$\scriptscriptstyle\blacksquare$}

\setlist[enumerate]{leftmargin=1em,labelsep=4.5pt}
\setlist[enumerate,1]{leftmargin=3em,label=(\arabic*)}
\setlist[enumerate,2]{label=(\roman*)}
\setlist[enumerate,3]{label=(\alph*)}

\setlist[description]{labelsep=6pt}

\hypersetup{
    setpagesize=false,
    colorlinks=true,
    citecolor=green!50!black,
    linkcolor=blue,
    urlcolor=cyan!70!black
}

